One-Shot Learning from a Demonstration with Hierarchical Latent Language

Humans have the capability, aided by the expressive compositionality of their language, to learn quickly by demonstration. They are able to describe unseen task-performing procedures and generalize their execution to other contexts. In this work, we introduce DescribeWorld, an environment designed to test this sort of generalization skill in grounded agents, where tasks are linguistically and procedurally composed of elementary concepts. The agent observes a single task demonstration in a Minecraft-like grid world, and is then asked to carry out the same task in a new map. To enable such a level of generalization, we propose a neural agent infused with hierarchical latent language--both at the level of task inference and subtask planning. Our agent first generates a textual description of the demonstrated unseen task, then leverages this description to replicate it. Through multiple evaluation scenarios and a suite of generalization tests, we find that agents that perform text-based inference are better equipped for the challenge under a random split of tasks.

==> tables/description_following.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{lllllll}
\toprule
\textbf{Task Completion (\%)} & \multicolumn{2}{l}{\textbf{LLP (Simple)}} & \multicolumn{2}{l}{\textbf{LLP}} & \multicolumn{2}{l}{\textbf{NVB}} \\
 &        \textbf{Valid} &     \textbf{Eval} &    \textbf{Valid} &     \textbf{Eval} &    \textbf{Valid} &     \textbf{Eval} \\
\textbf{Generalization Split}       &                       &                   &                   &                   &                   &                   \\
\midrule
\textbf{Random Split}               &      $74.28 \pm 6.40$ &  $73.60 \pm 6.46$ &  $73.82 \pm 4.65$ &  $73.37 \pm 4.44$ &  $\mathbf{83.12 \pm 1.62}$ &  $\mathbf{82.76 \pm 1.86}$ \\
\textbf{Hidden Subtask}             &      $77.41 \pm 5.32$ &  $10.52 \pm 4.46$ &  $78.33 \pm 4.19$ &  $10.19 \pm 4.84$ &  $\mathbf{85.77 \pm 1.53}$ &  $10.00 \pm 2.56$ \\
\textbf{Hidden Use Case}            &      $75.67 \pm 3.99$ &  $32.41 \pm 4.39$ &  $77.01 \pm 2.80$ &  $\mathbf{41.91 \pm 5.63}$ &  $\mathbf{84.84 \pm 1.02}$ &  $29.82 \pm 3.06$ \\
\textbf{Hidden Terrain Destination} &     $76.04 \pm 10.73$ &   $2.94 \pm 0.89$ &  $76.56 \pm 5.89$ &   $4.34 \pm 2.60$ &  $\mathbf{84.48 \pm 0.52}$ &   $\mathbf{8.69 \pm 0.94}$ \\
\bottomrule
\end{tabular}
    \caption{Task completion rate for groundtruth description-following}
    \label{tab:my_label}
\end{table*}

==> tables/full_pipeline_results.tex <==
\begin{table*}[]
    \centering
    \footnotesize
   \begin{tabular}{lllll}
\toprule
\textbf{Agent} &      \textbf{NVB} &      \textbf{LLD} &     \textbf{HLLP} &  \textbf{HLLP-SI} \\
\textbf{Generalization Split}       &                   &                   &                   &                   \\
\midrule
\textbf{Random Split}               &  $27.59 \pm 4.92$ &  $\mathbf{57.54 \pm 3.60}$ &  $50.48 \pm 8.12$ &  $54.26 \pm 2.88$ \\
\textbf{Hidden Subtask}             &   $\mathbf{2.38 \pm 0.76}$ &   $0.14 \pm 0.09$ &   $0.09 \pm 0.09$ &   $0.14 \pm 0.10$ \\
\textbf{Hidden Use Case}            &   $3.04 \pm 1.04$ &  $10.98 \pm 1.52$ &  $14.70 \pm 2.32$ &  $\mathbf{15.91 \pm 2.21}$ \\
\textbf{Hidden Terrain Destination} &   $3.59 \pm 1.35$ &   $4.38 \pm 0.09$ &   $4.19 \pm 0.42$ &   $\mathbf{6.87 \pm 0.75}$ \\
\bottomrule
\end{tabular}
    \caption{Task completion rate for full demonstration-following pipeline }
    \label{tab:my_label}
\end{table*}

==> tables/huc_description_following_results.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{lllll}
\toprule
           & \textbf{Agent} & \textbf{LLP (Simple)} &       \textbf{LLP} &       \textbf{NVB} \\
subtask & task\_type &                       &                    &                    \\
\midrule
diamond house & \textbf{Overall} &      $32.78 \pm 8.71$ &  $35.91 \pm 10.03$ &   $29.47 \pm 3.82$ \\
           & Building on Terrain &      $22.00 \pm 8.40$ &   $28.35 \pm 6.01$ &   $22.93 \pm 5.69$ \\
           & Crafting &     $53.54 \pm 11.30$ &  $50.46 \pm 17.76$ &   $42.05 \pm 9.61$ \\
iron flooring & \textbf{Overall} &      $30.97 \pm 5.68$ &   $51.56 \pm 9.34$ &   $32.04 \pm 9.63$ \\
           & Building on Terrain &       $6.55 \pm 7.45$ &  $41.54 \pm 12.36$ &   $13.59 \pm 9.90$ \\
           & Crafting &      $68.42 \pm 7.75$ &   $66.94 \pm 5.96$ &  $60.33 \pm 10.01$ \\
make goldware & \textbf{Overall} &     $40.99 \pm 10.27$ &  $37.28 \pm 18.62$ &   $36.72 \pm 6.21$ \\
           & Building on Terrain &     $27.44 \pm 11.65$ &  $30.10 \pm 13.88$ &   $17.08 \pm 4.20$ \\
           & Crafting &     $50.88 \pm 10.82$ &  $42.52 \pm 22.36$ &  $51.05 \pm 10.74$ \\
pig shrine & \textbf{Overall} &      $27.70 \pm 5.74$ &   $40.12 \pm 2.80$ &   $22.46 \pm 6.75$ \\
           & Building on Terrain &      $20.83 \pm 3.99$ &   $32.59 \pm 3.81$ &   $19.93 \pm 5.89$ \\
           & Crafting &      $39.57 \pm 9.26$ &   $53.12 \pm 3.30$ &   $26.82 \pm 9.39$ \\
\bottomrule
\end{tabular}
    \caption{Task completion rate for groundtruth description following under Hidden Use Case generalization split}
    \label{tab:huc_description_following}
\end{table*}

==> tables/huc_full_pipeline_results.tex <==
\begin{table*}[t!]
    \centering
\begin{tabular}{llllll}
\toprule
     & \textbf{Agent} &       \textbf{NVB} &       \textbf{LLD} &      \textbf{HLLP} &   \textbf{HLLP-SI} \\
split & subtask &                    &                    &                    &                    \\
\midrule
terrain & diamond house &    $5.33 \pm 5.58$ &  $84.00 \pm 10.11$ &  $77.33 \pm 21.40$ &  $89.33 \pm 10.11$ \\
     & iron flooring &  $33.33 \pm 33.33$ &   $94.67 \pm 8.69$ &   $69.33 \pm 7.60$ &   $90.67 \pm 7.60$ \\
     & make goldware &  $21.33 \pm 11.93$ &  $89.33 \pm 11.16$ &  $56.00 \pm 31.83$ &  $92.00 \pm 11.93$ \\
     & none &   $25.09 \pm 2.63$ &   $63.51 \pm 3.92$ &   $52.86 \pm 4.07$ &   $63.48 \pm 3.09$ \\
     & pig shrine &  $57.33 \pm 21.40$ &  $46.67 \pm 34.32$ &  $64.00 \pm 11.16$ &  $72.00 \pm 10.95$ \\
eval & diamond house &    $0.14 \pm 0.09$ &   $17.09 \pm 4.18$ &   $23.57 \pm 5.89$ &   $29.38 \pm 6.84$ \\
     & iron flooring &    $2.23 \pm 1.14$ &   $14.47 \pm 3.02$ &   $20.32 \pm 3.91$ &   $18.54 \pm 2.69$ \\
     & make goldware &    $1.82 \pm 1.83$ &    $6.49 \pm 1.21$ &    $5.48 \pm 3.46$ &    $7.53 \pm 1.46$ \\
     & pig shrine &    $8.53 \pm 3.63$ &    $2.23 \pm 0.62$ &    $3.19 \pm 0.95$ &    $2.07 \pm 0.85$ \\
\bottomrule
\end{tabular}
    \caption{Task completion rate for demonstration following under hidden procedural use case split}
    \label{tab:huc_full}
\end{table*}

==> tables/rs_description_following_results.tex <==
\begin{table*}[]
    \centering
    \small
   \begin{tabular}{lllllll}
\toprule
\textbf{split} & \multicolumn{3}{l}{terrain} & \multicolumn{3}{l}{eval} \\
\textbf{agent} & \textbf{LLP (Simple)} &      \textbf{LLP} &      \textbf{NVB} & \textbf{LLP (Simple)} &      \textbf{LLP} &      \textbf{NVB} \\
\textbf{Category}   &                       &                   &                   &                       &                   &                   \\
\midrule
Building on Terrain &      $60.40 \pm 9.73$ &  $63.97 \pm 5.35$ &  $74.00 \pm 2.34$ &      $58.97 \pm 9.56$ &  $63.09 \pm 4.78$ &  $73.26 \pm 2.85$ \\
Clearing Items      &      $79.86 \pm 4.70$ &  $81.57 \pm 8.11$ &  $94.82 \pm 2.10$ &      $78.35 \pm 7.86$ &  $82.01 \pm 6.20$ &  $94.80 \pm 1.86$ \\
Composite           &      $89.67 \pm 2.89$ &  $84.87 \pm 5.09$ &  $92.94 \pm 1.30$ &      $89.70 \pm 3.36$ &  $86.55 \pm 4.80$ &  $93.93 \pm 1.88$ \\
Crafting            &      $83.09 \pm 4.20$ &  $77.78 \pm 5.83$ &  $87.82 \pm 1.44$ &      $83.78 \pm 4.18$ &  $78.17 \pm 5.80$ &  $88.52 \pm 1.30$ \\
Navigation          &      $94.17 \pm 2.49$ &  $94.54 \pm 2.33$ &  $97.53 \pm 0.99$ &      $94.51 \pm 2.01$ &  $94.52 \pm 3.35$ &  $96.93 \pm 0.87$ \\
Ordered Navigation  &      $86.77 \pm 9.02$ &  $91.53 \pm 3.36$ &  $94.01 \pm 1.02$ &      $89.73 \pm 7.47$ &  $92.82 \pm 2.77$ &  $94.40 \pm 1.16$ \\
\bottomrule
\end{tabular}
    \caption{Task completion rate for groundtruth description following under random split, decomposed by task category.}
    \label{tab:my_label}
\end{table*}

==> tables/rs_full_pipeline_results.tex <==
\begin{table*}[]
    \centering
    \small
\begin{tabular}{lllllll}
\toprule
                       & \textbf{Agent} &      \textbf{NVB} &      \textbf{LLD} &      \textbf{HLLP} &   \textbf{HLLP-SI} &   \textbf{HLLP-NE} \\
\textbf{Split} & \textbf{Task Category} &                   &                   &                    &                    &                    \\
\midrule
\midrule \textbf{Valid} & \textbf{Overall} &  $25.96 \pm 4.67$ &  $72.70 \pm 3.14$ &   $61.99 \pm 5.38$ &   $57.96 \pm 5.92$ &   $49.19 \pm 8.98$ \\
                       & Crafting &  $44.55 \pm 7.84$ &  $85.23 \pm 1.89$ &   $80.49 \pm 6.12$ &   $77.25 \pm 4.25$ &  $65.21 \pm 10.93$ \\
                       & Building on Terrain &   $8.85 \pm 3.80$ &  $63.54 \pm 4.72$ &   $61.40 \pm 7.98$ &  $53.70 \pm 10.00$ &  $46.80 \pm 10.51$ \\
                       & Covering Terrain &   $4.07 \pm 3.32$ &  $67.52 \pm 5.10$ &    $4.88 \pm 4.76$ &    $7.32 \pm 4.83$ &    $1.76 \pm 1.62$ \\
                       & Navigation &  $55.17 \pm 3.44$ &  $35.07 \pm 2.11$ &   $29.57 \pm 1.89$ &   $31.56 \pm 2.54$ &   $34.39 \pm 2.65$ \\
                       & Composite &  $52.09 \pm 5.02$ &  $92.55 \pm 2.67$ &   $88.30 \pm 4.85$ &   $87.04 \pm 3.86$ &   $72.65 \pm 8.59$ \\
                       & Clearing Items &  $27.65 \pm 5.32$ &  $89.13 \pm 0.58$ &  $74.38 \pm 12.15$ &   $70.80 \pm 9.03$ &  $55.00 \pm 14.13$ \\
\midrule \textbf{Eval} & \textbf{Overall} &  $24.00 \pm 4.12$ &  $62.82 \pm 2.99$ &   $55.30 \pm 5.40$ &   $52.16 \pm 5.14$ &   $44.08 \pm 8.40$ \\
                       & Crafting &  $42.34 \pm 7.73$ &  $78.50 \pm 1.81$ &   $74.55 \pm 6.91$ &   $71.74 \pm 3.42$ &  $60.92 \pm 10.62$ \\
                       & Building on Terrain &   $6.89 \pm 2.74$ &  $51.80 \pm 4.91$ &   $52.39 \pm 7.32$ &   $46.05 \pm 8.73$ &   $39.25 \pm 9.32$ \\
                       & Covering Terrain &   $3.52 \pm 3.25$ &  $57.83 \pm 4.79$ &    $4.49 \pm 4.18$ &    $7.20 \pm 4.22$ &    $1.72 \pm 1.73$ \\
                       & Navigation &  $55.35 \pm 2.93$ &  $36.24 \pm 2.53$ &   $30.56 \pm 0.50$ &   $32.90 \pm 2.16$ &   $37.15 \pm 1.20$ \\
                       & Composite &  $46.89 \pm 5.51$ &  $83.43 \pm 1.57$ &   $83.01 \pm 4.22$ &   $82.41 \pm 4.27$ &  $68.04 \pm 10.69$ \\
                       & Clearing Items &  $17.25 \pm 4.31$ &  $40.92 \pm 1.41$ &   $35.25 \pm 7.97$ &   $36.67 \pm 7.19$ &   $27.35 \pm 8.27$ \\
\bottomrule
\end{tabular}
\begin{tabular}{llllllllll}
\toprule
                       & \textbf{Agent} & \multicolumn{2}{l}{\textbf{HLLP-NE}} & \multicolumn{2}{l}{\textbf{HLLP-SI}} & \multicolumn{2}{l}{\textbf{HLLP}} &      \textbf{NVB} &      \textbf{LLD} \\
                       & \textbf{Beam} &                  1 &                  5 &                 5 &                  1 &                 5 &                  1 &                -1 &                -1 \\
\textbf{Split} & \textbf{Task Category} &                    &                    &                   &                    &                   &                    &                   &                   \\
\midrule
\midrule \textbf{Valid} & \textbf{Overall} &   $49.17 \pm 8.98$ &  $49.65 \pm 10.29$ &  $58.57 \pm 4.13$ &   $57.96 \pm 5.92$ &  $61.77 \pm 1.71$ &   $61.97 \pm 5.38$ &  $25.96 \pm 4.67$ &  $72.70 \pm 3.14$ \\
                       & Crafting &  $65.18 \pm 10.93$ &  $65.88 \pm 12.51$ &  $77.37 \pm 5.09$ &   $77.25 \pm 4.26$ &  $79.12 \pm 2.21$ &   $80.45 \pm 6.12$ &  $44.55 \pm 7.84$ &  $85.23 \pm 1.89$ \\
                       & Building on Terrain &  $46.78 \pm 10.52$ &  $47.34 \pm 12.05$ &  $54.75 \pm 6.00$ &  $53.70 \pm 10.00$ &  $60.91 \pm 4.83$ &   $61.39 \pm 7.99$ &   $8.85 \pm 3.80$ &  $63.54 \pm 4.72$ \\
                       & Covering Terrain &    $1.77 \pm 1.63$ &    $1.76 \pm 1.87$ &   $7.81 \pm 2.84$ &    $7.32 \pm 4.84$ &   $8.36 \pm 7.04$ &    $4.88 \pm 4.76$ &   $4.07 \pm 3.32$ &  $67.52 \pm 5.10$ \\
                       & Navigation &   $34.38 \pm 2.65$ &   $34.39 \pm 3.06$ &  $31.45 \pm 2.81$ &   $31.56 \pm 2.54$ &  $28.39 \pm 0.89$ &   $29.57 \pm 1.89$ &  $55.17 \pm 3.44$ &  $35.07 \pm 2.11$ \\
                       & Composite &   $72.65 \pm 8.58$ &   $73.72 \pm 9.53$ &  $87.69 \pm 4.65$ &   $87.04 \pm 3.86$ &  $87.78 \pm 3.70$ &   $88.30 \pm 4.85$ &  $52.09 \pm 5.02$ &  $92.55 \pm 2.67$ \\
                       & Clearing Items &  $55.01 \pm 14.14$ &  $52.75 \pm 15.25$ &  $73.09 \pm 8.71$ &   $70.78 \pm 9.01$ &  $80.29 \pm 0.82$ &  $74.38 \pm 12.15$ &  $27.65 \pm 5.32$ &  $89.13 \pm 0.58$ \\
\midrule \textbf{Eval} & \textbf{Overall} &   $44.07 \pm 8.42$ &    $30.16 \pm nan$ &   $52.46 \pm nan$ &   $52.16 \pm 5.14$ &   $53.06 \pm nan$ &   $55.28 \pm 5.41$ &  $24.00 \pm 4.12$ &  $62.82 \pm 2.99$ \\
                       & Crafting &  $60.91 \pm 10.64$ &    $43.28 \pm nan$ &   $71.52 \pm nan$ &   $71.74 \pm 3.42$ &   $73.57 \pm nan$ &   $74.52 \pm 6.91$ &  $42.34 \pm 7.73$ &  $78.50 \pm 1.81$ \\
                       & Building on Terrain &   $39.24 \pm 9.34$ &    $23.95 \pm nan$ &   $47.06 \pm nan$ &   $46.05 \pm 8.73$ &   $47.78 \pm nan$ &   $52.38 \pm 7.33$ &   $6.89 \pm 2.74$ &  $51.80 \pm 4.91$ \\
                       & Covering Terrain &    $1.72 \pm 1.73$ &     $0.22 \pm nan$ &    $7.35 \pm nan$ &    $7.20 \pm 4.22$ &    $3.08 \pm nan$ &    $4.49 \pm 4.18$ &   $3.52 \pm 3.25$ &  $57.83 \pm 4.79$ \\
                       & Navigation &   $37.15 \pm 1.20$ &    $36.38 \pm nan$ &   $32.24 \pm nan$ &   $32.90 \pm 2.16$ &   $31.10 \pm nan$ &   $30.56 \pm 0.50$ &  $55.35 \pm 2.93$ &  $36.24 \pm 2.53$ \\
                       & Composite &  $68.04 \pm 10.69$ &    $51.55 \pm nan$ &   $81.02 \pm nan$ &   $82.41 \pm 4.27$ &   $82.69 \pm nan$ &   $82.99 \pm 4.22$ &  $46.89 \pm 5.51$ &  $83.43 \pm 1.57$ \\
                       & Clearing Items &   $27.35 \pm 8.27$ &    $15.25 \pm nan$ &   $39.33 \pm nan$ &   $36.67 \pm 7.19$ &   $39.33 \pm nan$ &   $35.25 \pm 7.97$ &  $17.25 \pm 4.31$ &  $40.92 \pm 1.41$ \\
\bottomrule
\end{tabular}

    \caption{Demonstration-following performance on random train split}
    \label{tab:rs_dem_following}
\end{table*}
